Linear Semantic Segmentation for Low-Resource Spoken Dialects

Semantic segmentation is a core component of discourse analysis, yet existing models are primarily developed and evaluated on high-resource written text, limiting their effectiveness on low-resource spoken varieties. In particular, dialectal Arabic exhibits informal syntax, code-switching, and weakly marked discourse structure that challenge standard segmentation approaches. In this paper, we introduce a new multi-genre benchmark (more than 1000 samples) for semantic segmentation in conversational Arabic, focusing on dialectal discourse. The benchmark covers transcribed casual telephone conversations, code-switched podcasts, broadcast news, and expressive dialogue from novels, and was annotated and validated by native Arabic annotators. Using this benchmark, we show that segmentation models performing well on MSA news genres degrade on dialectal transcribed speech. We further propose a segmentation model that targets local semantic coherence and robustness to discourse discontinuities, consistently outperforming strong baselines on dialectal non-news genres. The benchmark and approach generalize to other low-resource spoken languages.

==> Tables/evaluation_baselines1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[ht]
\centering
\small
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{llccccccccc}
\hline
\textbf{Type} & \textbf{Method} 
& \multicolumn{3}{c}{\textbf{OPUS News (MSA)}} 
& \multicolumn{3}{c}{\textbf{Rewayat (GL)}} 
& \multicolumn{3}{c}{\textbf{MGB-5 (MR)}} \\ \cline{3-11}
 &  & F1($\uparrow$) & Pk($\downarrow$) & WD($\downarrow$) & F1($\uparrow$) & Pk($\downarrow$) & WD($\downarrow$) & F1($\uparrow$) & Pk($\downarrow$) & WD($\downarrow$) \\ \hline
\multirow{4}{*}{Unsupervised}
  & TextTiling          & 0.56 & 0.45 & 0.49 & 0.51 & 0.48 & 0.49 & 0.50 & 0.55 & 0.71 \\	
  & AraTextTiling       & 0.55 & 0.40 & 0.42 & 0.54 & 0.42 & 0.44 & 0.50 & 0.52 & 0.57 \\
  & C99                 & 0.53 & 0.44 & 0.47 & 0.46 & 0.47 & 0.55 & 0.45 & 0.55 & 0.67 \\
  & ArabC99             & 0.56 & 0.41 & 0.43 & 0.52 & 0.44 & 0.48 & 0.49 & 0.53 & 0.60 \\ \hline				
\multirow{2}{*}{Embeddings}
  & TeT+CLS MARBERTv2   & 0.60 & 0.35 & 0.37 & \textbf{0.56} & \textbf{0.40} & \textbf{0.41} & \textbf{0.51} & 0.55 & 0.60 \\
  & TeT+CLS EmbeddingGemma & \textbf{0.62} & \textbf{0.34} & \textbf{0.36} & 0.55 & 0.41 & 0.43 & 0.51 & 0.56 & 0.61 \\ \hline
Supervised
  & SaT                 & 0.61 & 0.40 & 0.50 & 0.27 & 0.56 & 0.90 & 0.49 & 0.50 & 0.63 \\ \hline
\multirow{3}{*}{LLMs}
  & ALLaM-7B-Instruct   & 0.57 & 0.44 & 0.51 & 0.52 & 0.50 & 0.58 & 0.47 & 0.58 & 0.71 \\
  & Fanar-1-9B-Instruct   & 0.59 & 0.38 & 0.46 & 0.51 & 0.46 & 0.57 & 0.51 & 0.51 & 0.54 \\
  & Nile-Chat-12B               & 0.58 & 0.41 & 0.45 & 0.55 & 0.43 & 0.45 & 0.51 & 0.53 & 0.57 \\
  & Gemma3-4B               & 0.50 & 0.52 & 0.59 & 0.54 & 0.50 & 0.54 & 0.54 & 0.52 & 0.65 \\
  & \textit{Finetuned Gemma3-4B}  & 0.52 & 0.41 & 0.42 & 0.48 & 0.42 & 0.42 & 0.52 & \textbf{0.41} & \textbf{0.41} \\ \hline
\end{tabular}
\caption{Segmentation performance across news (Modern Standard Arabic), novels (Gulf), broadcast shows (Moroccan Arabic).}
\label{tab:segmentation_results}
\end{table*}


==> Tables/evaluation_baselines2.tex <==
\begin{table*}[ht]
\centering
\small
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{llccccccccc}
\hline
\textbf{Type} & \textbf{Method} 
& \multicolumn{3}{c}{\textbf{\shortstack{LDC Conversations\\(GL/IQ/LV)}}} 
& \multicolumn{3}{c}{\textbf{Podcasts (CS)}} 
& \multicolumn{3}{c}{\textbf{Poems (CA)}} \\ \cline{3-11}
 &  & F1($\uparrow$) & Pk($\downarrow$) & WD($\downarrow$) & F1($\uparrow$) & Pk($\downarrow$) & WD($\downarrow$) & F1($\uparrow$) & Pk($\downarrow$) & WD($\downarrow$) \\ \hline
\multirow{4}{*}{Unsupervised}
  & TextTiling        & 0.49 & 0.57 & 0.71 & 0.52 & 0.51 & 0.62 & 0.44 & 0.52 & 0.53 \\
  & AraTextTiling     & 0.53 & 0.48 & 0.56 & 0.56 & 0.42 & 0.47 & 0.45 & 0.52 & 0.53 \\
  & C99               & 0.50 & 0.52 & 0.60 & 0.53 & 0.46 & 0.52 & 0.45 & 0.49 & 0.54 \\
  & ArabC99           & 0.52 & 0.51 & 0.57 & 0.56 & 0.44 & 0.49 & 0.45 & 0.50 & 0.52 \\ \hline			
\multirow{2}{*}{Embeddings}
  & TeT+CLS MARBERTv2     & \textbf{0.54} & 0.48 & 0.57 & 0.56 & 0.43 & 0.49 & 0.48 & 0.50 & 0.51 \\
  & TeT+CLS EmbeddingGemma & 0.53 & 0.50 & 0.58 & \textbf{0.58} & \textbf{0.41} & 0.45 & 0.46 & 0.51 & 0.52 \\ \hline
Supervised
  & SaT               & 0.39 & 0.55 & 0.81 & 0.51 & 0.45 & 0.58 & 0.40 & 0.49 & 0.70 \\ \hline
\multirow{3}{*}{LLMs}
  & ALLaM-7B-Instruct   & 0.49 & 0.57 & 0.75 & 0.54 & 0.47 & 0.60 & 0.47 & 0.50 & 0.57 \\
  & Fanar-1-9B-Instruct   & 0.49 & 0.54 & 0.67 & 0.56 & 0.46 & 0.55 & \textbf{0.51} & \textbf{0.47} & 0.51 \\
  & Nile-Chat-12B       & 0.52 & 0.56 & 0.67 & 0.56 & 0.44 & 0.49 & 0.48 & 0.51 & 0.53 \\
  & Gemma3-4B           & 0.51 & 0.48 & 0.51 & 0.50 & 0.46 & 0.54 & 0.44 & 0.50 & 0.60 \\
  & \textit{Finetuned Gemma3-4B}& 0.52 & \textbf{0.38} & \textbf{0.38} & 0.49 & 0.43 & \textbf{0.43} & 0.49 & 0.48 & \textbf{0.48} \\ \hline
\end{tabular}
\caption{Segmentation performance across spontaneous conversations (Gulf/Iraqi/Levantine), podcasts (Code Switching, Gulf-English), poems (Classical Arabic).}
\label{tab:segmentation_ldc_podcast_poems}
\end{table*}

